Advancements in Traffic Processing Using Programmable Hardware Flow Offload

The exponential growth of data traffic and the increasing complexity of networked applications demand effective solutions capable of passively inspecting and analysing the network traffic for monitoring and security purposes. Implementing network probes in software using general-purpose operating systems has been made possible by advances in packet-capture technologies, such as kernel-bypass frameworks, and by multi-queue adapters designed to distribute the network workload in multi-core processors. Modern SmartNICs, in addition, have introduced stateful mechanisms to associate actions to network flows such as forwarding packets or updating traffic statistics for an individual flow. In this paper, we describe our experience in exploiting those functionalities in a modern network probe and we perform a detailed study of the performance characteristics under different scenarios. Compared to pure CPU-based solutions, SmartNICs with flow-offload technologies provide substantial benefits when implementing forwarding applications. However, the main limitation of having to keep large flow tables in the host memory remains largely unsolved for realistic monitoring and security applications.

==> additional.tex <==
\bibitem{b1} M. Sheeraz, H. Durad, S. Tahir, H. Tahir, S. Saeed, A.M. Almuhaideb,
``Advancing Snort IPS to Achieve Line Rate Traffic Processing for Effective Network Security Monitoring'',
IEEE Access, 2024.

\bibitem{b2} Q. Zhang, N. Ansari, Z. Zhu,
``Adaptive SmartNIC Offloading for Unleashing the Performance of Protocol-Oblivious Forwarding'',
IEEE Internet of Things Journal, 2022.



\bibitem{b4} S. Panda, et al., ``SmartWatch: Accurate traffic analysis and flow-state tracking for intrusion prevention using SmartNICs'', Proceedings of the 17th International Conference on Emerging Networking, 2021.





\bibitem{b7} C.E. Leiserson, N.C. Thompson, J.S. Emer, B.C. Kuszmaul, B.W. Lampson, D. Sanchez,
``There's plenty of room at the Top: What will drive computer performance after Moore's law?'',
Science, 2020

\bibitem{b8} Dally, William J., Yatish Turakhia, and Song Han,
``Domain-specific hardware accelerators'',
Communications of the ACM 63.7, 2020

\bibitem{b9} Hanford, Nathan, et al,
``A survey of end-system optimizations for high-speed networks'',
ACM Computing Surveys (CSUR) 51.3, 2018

\bibitem{b10} Y. Le, H. Chang, S. Mukherjee, L. Wang, A. Akella, M.M. Swift, T.V. Lakshman,
``UNO: Uniflying host and smart NIC offload for flexible packet processing'',
Proceedings of the 2017 Symposium on Cloud Computing, 2017

\bibitem{b11} P. Rygielski, M. Seliuchenko, S. Kounev, M. Klymash,
``Performance Analysis of SDN Switches with Hardware and Software Flow Tables'',
VALUETOOLS, 2016

\bibitem{b12} D. Vodák, K. Vojanec, J. Šuráň,
``What RTE flow rules can your NIC offload?'',
DPDK Userspace Summit, 2022

==> notes.tex <==
\section{Case Studies}

\subsection{Traffic Monitoring}

Passive

$\ldots$

After analyzing the initial packets of a network communication, and once the application protocol and metadata have been detected, the classifier can offload the flow to the adapter. Subsequent packets for the offloaded flow are processed by the adapter, which updates flow metadata (packets and bytes counters). Flow updates are periodically sent to the software. This improves performance and reduces CPU usage.

$\ldots$

\subsection{IDS/IPS Acceleration}

Inline (unidirectional)

$\ldots$

\subsection{Layer-7 Traffic Policing}

Inline (bidirectional)

$\ldots$

\section{Adapter Under Test}

The adapter used for the evaluation is a Napatech NT200A02. This adapter is using PCIe 3, supporting up to 100 Gbps in and 100 Gbps out.
The flow table offload support on this adapter, also known as Flow Manager, has room for 140 million flows with a learning rate of up to 1 million flows per second when using a single stream, 3 million flows per second maximum when using multiple streams.

\subsection{Capacity of the Hardware Flow Table}

When the flow table capacity is reached, unhandled packets are forwarded to the host: software fallback.

$\ldots$
